VerlTool: Towards Holistic Agentic Reinforcement Learning with Tool Use

Reinforcement Learning with Verifiable Rewards (RLVR) has demonstrated success in enhancing LLM reasoning capabilities, but remains limited to single-turn interactions without tool integration. While recent Agentic Reinforcement Learning with Tool use (ARLT) approaches have emerged to address multi-turn tool interactions, existing works develop task-specific codebases that suffer from fragmentation, synchronous execution bottlenecks, and limited extensibility across domains. These inefficiencies hinder broader community adoption and algorithmic innovation. We introduce VerlTool, a unified and modular framework that addresses these limitations through systematic design principles. VerlTool provides four key contributions: (1) upstream alignment with VeRL ensuring compatibility and simplified maintenance, (2) unified tool management via standardized APIs supporting diverse modalities including code execution, search, SQL databases, and vision processing, (3) asynchronous rollout execution achieving near 2$\times$ speedup by eliminating synchronization bottlenecks, and (4) comprehensive evaluation demonstrating competitive performance across 6 ARLT domains. Our framework formalizes ARLT as multi-turn trajectories with multi-modal observation tokens (text/image/video), extending beyond single-turn RLVR paradigms. We train and evaluate models on mathematical reasoning, knowledge QA, SQL generation, visual reasoning, web search, and software engineering tasks, achieving results comparable to specialized systems while providing unified training infrastructure. The modular plugin architecture enables rapid tool integration requiring only lightweight Python definitions, significantly reducing development overhead and providing a scalable foundation for tool-augmented RL research. Our code is open-sourced at https://github.com/TIGER-AI-Lab/verl-tool.

==> sections/code_design.tex <==
\section{Code Design}
\input{tables/tool_design}



==> tables/swe.tex <==
\begin{table}[!htbp]
\centering
\small
\caption{Results of VT-SWE on SWE-Verified Benchmark. Experiment details in ~\autoref{subsec:swe_details}.}
\label{tab:res_swe}
\begin{tabular}{lc}
\toprule
\textbf{Model} & \textbf{SWE-Verified Score} \\
\midrule
\multicolumn{2}{c}{\textit{\textbf{OpenHands Scaffold}}} \\
\midrule
Qwen3-8B             & 3.6 \\
OpenHands-7B-Agent             & 11.0 \\
\hdashline
\textit{SkyRL-v0} \citep{cao2025skyrl} \\
\quad Qwen3-8B Based & 9.4 \\
\quad OpenHands-7B-Agent Based & 14.6 \\
\midrule
\multicolumn{2}{c}{\textit{\textbf{R2E Gym Scaffold}}} \\
\midrule
Qwen3-8B             & 10.4 \\
\hdashline
\textit{VT-SWE (Qwen3-8B Based)} \\
\quad +GRPO & \textbf{19.5} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/tool_design.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c|c}
\toprule
\textbf{BaseTool (Template)} & \textbf{PythonCodeTool (Implementation)} \\
\midrule
\begin{minipage}{0.48\textwidth}
\begin{lstlisting}[style=python, basicstyle=\ttfamily\tiny]
@register_tool
class BaseTool:
    tool_type = __name__
    def __init__(self, num_workers=4):
        self.num_workers = num_workers
        self.env_cache = {}

    def parse_action(self, action:str):
        # parse llm-generated action and determine if match
        parsed_action = ...
        valid = True # invoke this tool if match (True), 
        return parsed_action, valid

    def load_env(self, trajectory_id):
        env = ...
        return env
    
    def save_env(self, trajectory_id, env):
        ...
    
    def update_env(self, trajectory_id, env, **kwargs):
        ...

    def conduct_action(self, trajectory_id:str, action:str, extra_field:dict):
        parsed_action, is_valid = self.parse_action(action)
        # load current env
        env = self.load_env(trajectory_id)

        # get observation from parsed_action
        observation = ...

        done = True # if ending this trajectory 

        # update and save the current env
        self.update_env(trajectory_id, env, parsed_action, is_valid, extra_field, observation)
        self.save_env(trajectory_id, env)
        
        return observation, done, is_valid
\end{lstlisting}
\end{minipage}
&  
\begin{minipage}{0.48\textwidth}
\begin{lstlisting}[style=python, basicstyle=\ttfamily\tiny]
from .base import BaseTool, register_tool

def execute_python(code:str, timeout:int=60):
    # use subprocess to launch a Python execution
    ...
    return stdout, stderr, has_error
    
@register_tool
class PythonCodeTool(BaseTool):
    tool_type = "python_code"

    def parse_action(self, action:str):
        # Try to find Python code in various formats
        all_valid_python_code = re.findall(r"<python>(.*?)</python>", action, re.DOTALL)
        
        if len(all_valid_python_code) == 0:
            return "", False
        # use all the code blocks
        parsed_code = "\n".join([code.strip() for code in all_valid_python_code])
        return parsed_code, True

    def conduct_action(self, trajectory_id:str, action:str, extra_field:dict):
        parsed_action, is_valid = self.parse_action(action)
        # load current env
        env = self.load_env(trajectory_id)

        # get observation from parsed_action
        stdout, stderr, has_error = execute_code(parsed_code)
        observation = stdout + "\n" + stderr
        
        done = False # do not end until the llm reaches max turns or max length

        # update and save the current env
        self.update_env(trajectory_id, env, parsed_action, is_valid, extra_field, observation)
        self.save_env(trajectory_id, env)
        
        return observation, done, is_valid
\end{lstlisting}
\end{minipage}
\\
\bottomrule
    \end{tabular}
    \caption{Example of adding a new tool in \ours framework. Users can only focus on implementing these interface functions, while \ours will take care of the concurrent tool-calling and model training.}
    \label{tab:placeholder}
\end{table}
